Bilateral Trade with Correlated Values

We study the bilateral trade problem where a seller owns a single indivisible item, and a potential buyer seeks to purchase it. Previous mechanisms for this problem only considered the case where the values of the buyer and the seller are drawn from independent distributions. In this paper, we study bilateral trade mechanisms when the values are drawn from a joint distribution. We prove that the buyer-offering mechanism guarantees an approximation ratio of $\frac e {e-1} \approx 1.582$ to the social welfare even if the values are drawn from a joint distribution. The buyer-offering mechanism is Bayesian incentive compatible, but the seller has a dominant strategy. We prove the buyer-offering mechanism is optimal in the sense that no Bayesian mechanism where one of the players has a dominant strategy can obtain an approximation ratio better than $\frac e {e-1}$. We also show that no mechanism in which both sides have a dominant strategy can provide any constant approximation to the social welfare when the values are drawn from a joint distribution. Finally, we prove some impossibility results on the power of general Bayesian incentive compatible mechanisms. In particular, we show that no deterministic Bayesian incentive-compatible mechanism can provide an approximation ratio better than $1+\frac {\ln 2} 2\approx 1.346$.

==> notations.tex <==
\renewcommand{\d}[1]{\ensuremath{\, d{#1}}}

\newcommand{\welfare}[2]{{#1}_{#2}} % the welfare of a mechanism 
\newcommand{\gft}[2]{{#1}_{#2}} % the gains from trade of a mechanism 

\newcommand{\distributionlbbp}{\mathcal{F}} % the distribution of the buyer-pricing lower bound 
\newcommand{\distributionlbonesided}{\mathcal{F}^{k,\varepsilon}} % the distribution of the one-sided mechanisms lower bound 

\newcommand{\distributionlbonesidedcdfs}{{\mathcal{F}_{{s|b}}^{k, \varepsilon}}} % the cdf of the marginal distribution of the seller in the lower bound of one-sided mechanisms

\newcommand{\distributionlbonesidedpdfs}{{f_{{s|b}}^{k, \varepsilon}}} % the pdf of the marginal distribution of the seller in the lower bound of one-sided mechanisms

\newcommand{\distributionlbdsic}[1]{\mathcal{F}_{#1}} % the distribution of the DSIC lower bound

\newcommand{\distributionlbdsicpdf}[1]{{p}_{#1}} % the pdf of the buyer in the DSIC lower bound

\newcommand{\prbuyervalue}[1]{x_{#1}} % the probability that the buyer's value is some b. 


\definecolor{tradepossiblecolor}{HTML}{FFA812}
\newcommand{\tradepossiblecolorname}{orange }

% \newcommand{\positiveprobcolor}{violet!70}
\newcommand{\thsbuyercolor}{yellow}
\newcommand{\thsbuyercolorname}{yellow }
\newcommand{\thssellercolor}{violet}
\newcommand{\thssellercolorname}{ purple }


